Evaluation of Field-Aware Neural Ranking Models for Recipe Search

Explicitly modelling field interactions and correlations in complex document structures has recently gained popularity in neural document embedding and retrieval tasks. Although this requires the specification of bespoke task-dependent models, encouraging empirical results are beginning to emerge. We present the first in-depth analyses of non-linear multi-field interaction (NL-MFI) ranking in the cooking domain in this work. Our results show that field-weighted factorisation machines models provide a statistically significant improvement over baselines in recipe retrieval tasks. Additionally, we show that sparsely capturing subsets of field interactions based on domain knowledge and feature selection heuristics offers significant advantages over baselines and exhaustive alternatives. Although field-interaction aware models are more elaborate from an architectural basis, they are often more data-efficient in optimisation and are better suited for explainability due to mirrored document and model factorisation.

==> sections/02_introduction.tex <==
\section{Introduction}

%Recommender Systems (RS) are important research field. Some RSs share key fundamentals with Information Retrieval (IR) and there is clear convergence between these fields of research~\cite{belkin1992information}. The convergence is such that in some cases retrieval models can be learned from recommendation data~\cite{Zamani2020} or a RecSys problem reformulated as a IR task~\usepackage{Costa10} or adapting IR models to social network recommendations~\cite{Sanz-Cruzado19}.

Cooking has become a vital daily routine for hundreds of millions of people. Under pandemic restrictions it has brought family cohesion and mental health support for many people globally. 

Cooking recipes are rich documents containing a wealth of  fields, such as classic title, body, the anchor text from incoming hyperlinks, but also images, comments and the query text used to find the recipe.

% Field dependencies have traditionally been seen as not critical for some search applications \cite{mitra2019incorporating,sarvi2020comparison}. Although multiple fields may contain complementary information. 

% This intuition is exploited by traditional information retrieval (IR) techniques where field interactions are explicitly considered and deemed to be important~\cite{Robertson2004}. A number of techniques have been explored to represent these interactions and their impact in IR~\cite{piwowarski2003machine, svore2009machine, kim09prob, kim2012field}.

Until recently, deep neural ranking models (NRMs) tended to consider a single source of document description, such as document title~\cite{huang2013learning} or body text~\cite{Dehghani2017nrmweak}. Interactions between fields have recently started to be considered in NRMs. 

Field relevance modelling is usually conceived in two different ways: 1) from fields represented independently and then combined to create a weighted mode~\cite{Binsheng18field-based-relevance, DBLP:journals/corr/abs-1711-09174} or 2) directly from the entire document and using a relevance model to score fields~\cite{Binsheng18field-based-relevance}.

%\cite{DBLP:journals/corr/abs-1711-09174} show how neural models can deal with multiple heterogeneous document fields by taking a representation-based-like approach, which learns query-field or field relevance interactions and concatenates feature vectors to aggregate scores.

While~\cite{DBLP:journals/corr/abs-1711-09174} explicitly learn query-field interactions, no prior works have explicitly explored the nature of field-to-field interactions to better understand their inter-relations. Simple combinations of relevance on each field~\cite{Binsheng18field-based-relevance} or field representation concatenations~\cite{DBLP:journals/corr/abs-1711-09174} have been used. Like in attention models for natural language processing, it may be that some interactions between fields are non linear in nature. The order of field-to-field non linearities and their impact on ranking performance is unexplored.

We evaluate our models in the context of web search, using
the queries sampled from the Cookpad's`\footnote{http://www.cookpad.com} search logs. We study multiple field combinations to understand if more complex non-linear combinations can have an impact on retrieval performance.

In order to assess the robustness of our findings, this work also explores the impact of the architectural model employed for the information retrieval task.

In this work, we study the following research hypotheses:

\begin{itemize}
    \item \textbf{H1} Non-linearities in field-to-field interactions have an impact in ranking performance. Feature concatenation may not be the most effective mechanism to unveil these dependencies, even though it is the most widely used way of amalgamating multiple field information. 
    \item \textbf{H2} Specific field-to-field interactions affect performance (beyond query-field interactions).
    \item \textbf{H3} The importance of field interactions are dependent on the neural architecture employed for the analysis.
\end{itemize}

Our experiments validate all these hypotheses, and investigate
the effectiveness of our overall exploration of field interactions.
\todo{Do we need he classic paragraph that summarises the rest of the paper or can we skip it for a short paper}


%We take inspiration from interaction-based models, which learn representations by interacting query and document from the first layer, and explore the importance of query-field interactions and field-to-field interactions. 

%  Many variants have been proposed in both architecture to better model relevance between query and document, but they were mainly designed for single-field document ranking. 


==> sections/03_related_work.tex <==
\section{Related Work}
\label{sec:related_work}

%\subsection{Retrieval with Multiple Fields}

% Using structural information to improve document retrieval
% is a mature topic in information retrieval. Wilkinson~\cite{Wilkinson1994} proposed
% several ways to to combine section-level and document-level evidence, such as taking the maximum section score, or a weighted sum of section scores, and then combining with a document-level score. 

% The classic BM25 and BM25F already used information from multiple fields ~\cite{robertson1995okapi,Robertson2004}. Other approaches built on this idea without resorting to a linear combination of per-field scores: like, for instance, Bayesian networks~\cite{piwowarski2003machine}, LambdaBM25~\cite{svore2009machine} (based on LambdaRank~\cite{burges2007learning}), language modeling framework~\cite{Ogilvie03known}, probabilistic models~\cite{kim09prob}, or feedback weighted field relevance~\cite{kim2012field}.
%Robertson et al.} extended the original BM25 model to create the BM25F model, which combines frequency information across fields on a per-term basis and then computes a retrieval score using a balanced approach.

% Wilkinson proposed several heuristic methods of combining section-level and document-level evidence, such as taking the maximum section score or taking a weighted sum of section scores \cite{wilkinson1994effective}.



%\subsection{Neural Networks for Ranking}

While there are many works focusing on the application of neural models to information retrieval~\cite{MitraandCraswellNIR18},  most of them treat each document as a single instance of text (i.e., single field) disregarding semi-structured information in multiple fields. 

%However, documents often include information in a semi-structured format and multiple fields.  A few studies have discussed how to use evidence from structure to improve the performance of information retrieval systems. 

Neural Ranking Models for Fields (NRM-F; its naming is inspired by BM25F \cite{perez2010using}) is the seminal paper that discusses how neural models can deal with multiple document fields from an architectural perspective  \cite{DBLP:journals/corr/abs-1711-09174}. The work suggests that it is better to score the whole document jointly, rather than generate a per-field score and aggregate. 
% 
Its formulation for document representation learning function $\Phi_D$ is as follows:
$$
\Phi_{D}\left(F_{d}\right)=\Lambda_{D}\left(\Phi_{F_{1}}\left(F_{1}\right), \Phi_{F_{2}}\left(F_{2}\right), \cdots, \Phi_{F_{k}}\left(F_{k}\right)\right)
$$
where $\Phi_{F_{i}}$ denotes the mapping function for the field $F_i$ and $\Lambda_D$ is an aggregation function which consolodates representations learned for all the fields. In their formulation, $\Lambda_{D}$ is the concatenation function which combines the input vectors. A densely-connected a stack of layers outputs the final retrieval score.

In NRM-F, both query text and text fields are represented using a character $n$-gram hashing vector \cite{huang2013learning}, and a convolution layer is then employed to capture the dependency between terms.
% 
Although NRM-F explicitly learns query-field interactions, it does not distinctly consider field-to-field interactions. In this manner, it can learn about the relevance of each field, but not account for correlated field features. There is some existing work that investigates query-to-field interactions in these applications \cite{Binsheng18field-based-relevance}, but this work assumes that linear relationships between relevance models induced from each field. %NRM-F also exclusively focuses on query-field interactions (scoring the whole document jointly), but there may be other important field interactions to consider. 



% When designing a ranking model, several architecture decisions need to be made, such as representation-based vs. interaction-based, which field interactions to learn, how to aggregate scores, etc. These fundamental design decisions were not clearly justified in prior efforts and the impact of the chosen architectural model on ranking remains unclear.

As well as NRM-F, several other potential models can be extended to shine light on the value of complex field interaction modelling. Factorization Machines (FM) are one model type that are widely used supervised learning approach. These models effectively modeling of feature interactions, and interactions can be captured with arbitrary interaction functions, allowing for models that capture effect non-linear interactions between fields. 
% In FM, unseen feature interactions can be learned from other pairs. 
Field-weighted Factorization Machine (FwFM) are state-of-the-art among the shallow models for click-through-rate prediction~\cite{pan2018field}.

Many non model-based approaches for producing field-aware document representations exist. The classic BM25 heuristic, for example, has a field-aware varient called BM25F that is used information from multiple fields ~\cite{robertson1995okapi,Robertson2004}. Other approaches built on this idea without resorting to a linear combination of per-field scores: like, for instance, Bayesian networks~\cite{piwowarski2003machine}, LambdaBM25~\cite{svore2009machine} (based on LambdaRank~\cite{burges2007learning}), language modeling framework~\cite{Ogilvie03known}, probabilistic models~\cite{kim09prob}, or feedback weighted field relevance~\cite{kim2012field}.


==> sections/04_methodology.tex <==
\section{Methodology}

\subsection{Datasets}

% \subsubsection{MS MARCO Dataset}
% Microsoft has released a large web search dataset called MS MARCO \footnote{MS MARCO \url{https://microsoft.github.io/msmarco/}}. The documents consist of multiple fields. 

% \subsubsection{Recipe Search Dataset}

Cookpad\footnote{Cookpad \url{http://www.cookpad.com}} is the world's largest recipe community web service where users can publish and search for recipes. For the experiements described later, we consider recipe and search log data from Cookpad. 
% main subsets of data arise from Cookpad: recipe data and search logs.

Recipes consist of multiple fields and media types. We selected six fields for modelling: query, title, ingredients, description, country, and image. The title field is usually short and consists of 3.47 words on average. The ingredients field is a variable-sized set of texts since some recipes require more ingredients than others. The description is also a list of free text fields; some recipes have a surprisingly long description while there are recipes with virtually no description. The country field indicates the country in which the recipe was published. Recipes have a main image and several step images, but only the main image is used in the experiment since it captures the whole recipe, rather than capturing a specific step. 

Search events are tracked when a user clicks a recipe in the search results. Each log contains session ID, event time, retrieved recipe IDs, clicked recipe ID, and clicked position. The average number of words in a query is 2.25. A variety of query types arre found in the logs, including question-like queries such as `how to bake cake without oven' and `what is buttermilk'. Over 99\% of queries are `clean' with users specifically searching for ingredients, dishes, regions, etc. 
% account for less than 1\% of the queries. 
% This is different from the MS MARCO dataset in which queries are usually long and most of the queries are question-like queries.

% \begin{table}
%     \centering
%     \begin{tabular}{l|l|l}
%         \hline
%         Field & Type & Example \\
%         \hline
%         recipe\_id & Integer & 1 \\
%         title & String & Honey garlic chicken thighs \\
%         description & String & This recipe has always been my favorite \\
%         ingredients & String set & chicken, salt, crushed red chilli, ... \\
%         country & String & GB \\
%         \hline
%     \end{tabular}
%     \caption{The schema of recipe data}
%     \label{tab:schema_of_recipe_data}
% \end{table}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.54\textwidth]{images/words_in_fields.png}
%     \caption{Number of words in text fields in the Cookpad data}
%     \label{fig:words_in_fields}
% \end{figure}

% \begin{table}
%     \centering
%     \begin{tabular}{l|l|l}
%         \hline
%         Field & Type & Example \\
%         \hline
%         session\_id & Integer & 1 \\
%         query & String & hot dessert \\
%         recipe\_id & Integer & 1 \\
%         position & Integer & 1 \\
%         fetched\_recipe\_ids & String & 1,2,3,4,5,6 \\
%         \hline
%     \end{tabular}
%     \caption{The schema of search log in Cookpad}
%     \label{tab:schema_of_search_log}
% \end{table}

\subsection{Data Processing and Modeling}
\label{subsec:data processing and modeling}

\begin{figure}
     \centering
     \begin{subfigure}[b]{0.8\linewidth}
         \centering
         \includegraphics[width=\textwidth]{images/diagram_nrmf.png}
         \caption{NRM-F architecture.}
         \label{fig:diagram_of_nrmf}
     \end{subfigure}\\
     \begin{subfigure}[b]{0.8\linewidth}
         \centering
         \includegraphics[width=\textwidth]{images/diagram_fwfm_all.png}
         \caption{FwFM architecture}
         \label{fig:diagram_of_fwfm}
     \end{subfigure}
        \caption{Architecture of considered models.}
        \label{fig:architectures}
\end{figure}

Search logs are aggregated by session ID and query to form listwise data. Each result list is trimmed at the last clicked position in the list, and items above the position are treated as negatives, as they were examined by a user but not clicked. Regarding the text representation, we obtain fix-sized vectors under the assumption that terms are almost independent as observed earlier. We use the average of term vectors, which has been shown to perform similar or slightly better than recurrent units with significantly less training time \cite{DBLP:journals/corr/abs-1907-00937}. Countries are treated as a category and embedded into a latent space.  We employ an image embedding that is pre-trained on ImageNet \cite{imagenet_cvpr09}.

In order to test if field interactions affect ranking performance in an architecture-dependent manner, we focus on two architectural models: NRM-F~\cite{DBLP:journals/corr/abs-1907-00937} and FwFM~\cite{pan2018field} to examine how the choice of architecture affects effectiveness along with the concatenation model that concatenates all encoded features as baseline. Figure \ref{fig:architectures} show the diagrams of NRM-F (\ref{fig:diagram_of_nrmf}) and FwFM (\ref{fig:diagram_of_fwfm}) employed in our experiments. The characteristic differences of how fields are modelled, aggregated and distilled into scores are summarised in Table \ref{tab:differences_in_models}. Our experimentation will explore several novel configurations of both models that are described below. 





% \begin{figure}
%     \centering
%     \includegraphics[width=0.4\textwidth]{images/diagram_nrmf.png}
%     \caption{The diagram of our simplified NRM-F model}
%     \label{fig:diagram_of_nrmf}
%     % \vspace{-4mm}
% \end{figure}

% \begin{figure}
% \footnotesize
%     \centering
%     \includegraphics[width=0.4\textwidth]{images/diagram_nrmf.png}
%     \caption{The diagram of our FwFM model}
%     \label{fig:diagram_of_fwfm}
%     % \vspace{-8mm}
% \end{figure}

\begin{table}[H]
    \centering
    % \small
    \caption{Model and field interaction configurations of the two architectures evaluated in this work.}
    \begin{tabular}{lll}
        \toprule
        & NRM-F & FwFM \\
        \midrule
        First-order features & Not used & Used \\
        Interaction selection & Query-field & All \\
        Interaction representation & Hadamard product & Dot product \\
        Interaction aggregation & Concatenation & Weighted sum \\
        \bottomrule
    \end{tabular}
    \label{tab:differences_in_models}
\end{table}

We employ Normalised Discounted Cumulative Gain (NDCG) at 20 to evaluate models. The cuttoff of 20 was chosen since this is the number of recipes served per page. The loss is computed in a pairwise fashion. We evaluate performance on 10-fold cross validation data with pairwise T-tests with a (fairly stringent) threshold of significance set to $\alpha=0.01$. 

\subsection{Terminology}

By $1^{st}$ order interactions, we refer to features constructed taking individual fields into consideration. Hence, $2^{nd}$ order interactions are composites of pairs of features. By all interactions, we refer to models that include $1^{st}$ and $2^{nd}$ order features altogether. Query field interactions are just a specific type of $2^{nd}$ order features
% \begin{itemize}
%     \item First order
%     \item Second order
%     \item All interactions
%     \item Query-field 
%     \item Non-linear
%     \item Selected (?) 
% \end{itemize}


==> sections/05_experiments.tex <==

\section{Experiments}
All the experiments presented in this section are available on GitHub. 

% Removed for anonymous sumbission \footnote{\url{https://github.com/rejasupotaro/field-interactions-in-document-ranking}}.

\subsection{Query-to-field vs Field-to-field Interactions}
\label{subsec:q2ff2f}

% [NT: didn't really understand this, nor did I feel we justify it] Query-field interactions are considered to be important in document ranking, whereas recommendation models do not distinguish between context and item features. 
We gauge the effects of adding all feature interactions vs. focusing on query-field interactions only as follows.

\begin{itemize}
    \item \textbf{Concatenation (all)} Concatenate all features into a vector (as a baseline implementation).
    \item \textbf{NRM-F (all) / FwFM (all)}: Consider all feature interactions without distinguishing between query and fields.
    \item \textbf{NRM-F (query-field) / FwFM (query-field)}: Consider query-field interactions.
    % \item \textbf{FwFM (all)} : Consider all feature interactions without distinguishing between query and fields (as the original implementation).
    % \item \textbf{FwFM (query-field)}: Consider query-field interactions.
\end{itemize}

Table \ref{tab:rq2_result} shows the mean of the scores of the mentioned models. The models that learned query-field interactions outperformed models trained using all interactions in both NRM-F and FwFM. The results of `FwFM (query-field)' are the best, and its improvement over all others is statistically significant. 
% Table \ref{tab:rq2_p_values} shows these differences are statistically significant.

\begin{table}
    \centering
    \small
    \caption{Comparison of NRM-F-based and FM-based models on mean NDCG scores. $\dagger$ specifies statistically significant .}
    \begin{tabular}{ll}
        \toprule
        Model & NDCG@20 \\
        \midrule
        Concatenation model (all) & 0.643 \\
        NRM-F-based model (all) & 0.641 \\
        NRM-F-based model (query-field) & 0.652 \\
        FM-based model (all) &  0.661 \\
        FM-based model (query-field) & 0.667 $^\dagger$ \\
        \bottomrule
    \end{tabular}
    \label{tab:rq2_result}
    % % \vspace{-6mm}
\end{table}

Figure \ref{fig:rq2_boxplot} plots the NDCG scores on each validation data out of 10 splits. We can see that as well as having a higher median, the spread and inter-quartile range of this configuration is narrower. Given the statistical significance of the results, and the general improvements, these results add support for Hypothesis 1. 

% NT? The experiment also has shown that recommendation models could be used for ranking tasks as it is as FwFM outperformed the simplified NRM-F in this experiment. Besides, we can further improve performance by incorporating the properties of information retrieval into recommendation models.


\begin{figure}[h]
    \centering
    \includegraphics[width=0.8\linewidth]{images/experiment_1.pdf}
    \caption{NDCG scores for various model configurations.}
    \label{fig:rq2_boxplot}
\end{figure}




% \begin{table}
%     \centering
%     \begin{tabular}{l|c}
%         \hline
%         Pair & p-value \\
%         \hline
%         NRM-F (query-field) - NRM-F (all) & 0.030 \\
%         FwFM (query-field) - FwFM (all) & 0.502 \\
%         \hline
%     \end{tabular}
%     \caption{P-values of paired t-tests on each method}
%     \label{tab:rq2_p_values}
% \end{table}

% \subsection{Importance of Interactions beyond Query-Fields}
\subsection{Beyond Query-Field Interactions}

Subsection~\ref{subsec:q2ff2f} suggests some naturally leads to wondering whether other field interactions beyond query-field interactions can be identified.
% 
In this set of experiments, we employed the FwFM model, trained using $1^\text{st}$ and $2^\text{nd}$ order interactions (6 and 15 feature interactions respectively). FMs compute the scores for each field independently and sum them up to produce the final score. We trained the model regularly and extracted the individual feature scores on validation data.

Since the sum of the individual scores is the final score, we sort the features by their correlation with label, assuming that correlation is a proxy indicator of field importance. Then, we compare the performance of the following three models.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.4\textwidth]{images/rq4_output.png}
%     \caption{The distribution of the outputs of the FwFM model by label on validation data}
%     \label{fig:rq4_output}
% \end{figure}

Figure \ref{fig:rq4_corr} shows the correlations of the activation of fields by label. We can see that several interaction pairs are highly correlated with the labels. The highest (title-country) suggests that regionality and the category (captured through the title) are highly predictive for search re-ranking. It is likely that the correlations between these two fields capture regional preferences which results in the high value of this pair. Image has a low weight. This is somewhat surprising and a useful outcome of the experiment since \textit{a priori} image aesthetics were assumed to contribute highly to interactions due to their visual appeal. The low correlation on all image pairs indicates that image features (which are expensive to compute) may be dropped from models with limited consequences to metrics. 

We can use the correlation figure to select a sparse subset of interactions to capture. We make selections by choosing the feature pairs that are most correlated with click labels in the validation set, and Table 3 presents the results. This table shows that using the correlation table to specify model architectures can result in improved performance. Both `query-field' and `selected' offer a statistically significant improvement over `all' but with many fewer interactions modelled. Although the `query-field' results are higher, the `selected' option may be useful in scenarios without a query term (e.g. for social network feeds). These results offer evidence for accepting Hypothesis 2 on the value of the value of sparse interaction pairs is provided here. 
% shows the performance of the FwFMs with different features: the model with selected features did not outperform the model with query-field interactions.

\begin{figure}
    \centering
    \small
    \includegraphics[width=0.9\linewidth]{images/correlation.pdf}
    \caption{The correlation to the label of each feature. }
    \label{fig:rq4_corr}
\end{figure}

% These results suggest that the model cannot guess which recipe is more likely to be engaged with just by looking at a query. Also, correlation seems to be associated to the importance of the features. 

\begin{table}
    \centering
    \small
    \caption{The results for the interaction-oriented experiments. $\dagger$ indicates that performance improvement is statistically significant over unmarked rows.}
    \begin{tabular}{ll}
        \toprule
        Model & NDCG@20 \\
        \midrule
        FwFM (all) & 0.661 \\
        FwFM (selected) & 0.663 $^\dagger$ \\
        FwFM (query-field) & 0.667 $^\dagger$\\
        \bottomrule
    \end{tabular}
    \label{tab:rq4_result}
    % \vspace{-6mm}
\end{table}



\subsection{Non-Linear Field Interactions}

The original implementation of NRM-F does not use $1^\text{st}$ order field interactions. In this section, we explore the impact of $1^\text{st}$ order field interactions in performance. We compare NRM-F-based and FM-based models with different sets of features as follows:

\begin{itemize}
    \item {NRM-F ($2$)}: Use $2^\text{nd}$ order query-field interactions only (as the original implementation).
    \item {NRM-F ($1~\&~2$)}: Use $1^\text{st}$ order features along with $2^\text{nd}$ order query-field interactions.
    \item {FwFM ($2$)}: Use $2^\text{nd}$ order interactions only.
    \item {FwFM ($1~\&~2$)} : Use $1^\text{st}$ and $2^\text{nd}$ order interactions (as the original implementation).
\end{itemize}

\begin{table}
    \centering
    \caption{Comparison of models with different feature sets. 
    % `FM-based model ($1^\text{st}$ + $2^\text{nd}$)' with $1^\text{st}$ and $2^\text{nd}$ order interactions is statistically better than the alternatives, except for `NRM-F-based model ($2^\text{nd}$)'. However, if outlying datapoints are removed, `FM-based model ($1^\text{st}$ + $2^\text{nd}$)' out-performs all others. 
    }
    \begin{tabular}{lll}
        \toprule
        Model & Interactions & NDCG@20 \\
        \midrule
        NRM-F model & $2^\text{nd}$ & 0.652 \\
        NRM-F model & $1^\text{st}$ $\&$ $~2^\text{nd}$ & 0.650 \\
        FwFM model  & $2^\text{nd}$ & 0.645 \\
        FwFM model  & $1^\text{st}$ $\&$ $~2^\text{nd}$ & 0.661 $^\dagger$ \\
        \bottomrule
    \end{tabular}
    \label{tab:rq4_result}
    % \vspace{-6mm}
\end{table}

Table \ref{tab:rq4_result} shows the average NDCG scores for the above models. The results for the FwFM have not significantly changed, though they dipped slightly. However, the average results for the NRM-F based model have improved significantly over the baselines presented in Section \ref{subsec:q2ff2f}. Since including field interactions improved NRM-F, we believe evidednce for Hypothesis 2 is provided here. FwFM models are still the top-performing on this dataset, and `FwFM $1^\text{st}$ $\&$ $~2^\text{nd}$' is significantly better than the rest.
% It can be seen that there is no difference between NRM-F ($2^\text{nd}$) and NRM-F ($1^\text{st}$ + $2^\text{nd}$) while FwFM ($1^\text{st}$ + $2^\text{nd}$) significantly outperformed FwFM ($2^\text{nd}$) % (Table \ref{tab:rq3_p_values}), meaning that $1^\text{st}$ order features potentially improve effectiveness.


% \begin{figure}
%     \centering
%     \includegraphics[width=0.4\textwidth]{images/rq3_boxplot.png}
%     \caption{Comparison of the models trained with $2^\text{nd}$ order feature interactions vs. $1^\text{st}$ + $2^\text{nd}$ order feature interactions}
%     \label{fig:rq3_boxplot}
% \end{figure}

% \begin{table}
%     \centering
%     \begin{tabular}{l|c}
%         \hline
%         Pair & p-value \\
%         \hline
%         NRM-F ($2^\text{nd}$) - NRM-F ($1^\text{st}$ + $2^\text{nd}$) & 0.900 \\
%         FwFM ($2^\text{nd}$) - FwFM ($1^\text{st}$ + $2^\text{nd}$) & 0.001 \\
%         \hline
%     \end{tabular}
%     \caption{P-values of paired t-tests on each method}
%     \label{tab:rq3_p_values}
% \end{table}

% \begin{figure}
%     \centering
%     \includegraphics[width=0.4\textwidth]{images/rq4_boxplot.png}
%     \caption{Comparison of the impact of features used in FwFM}
%     \label{fig:rq4_boxplot}
% \end{figure}
